Scary Barbie: An Extremely Energetic, Long-Duration Tidal Disruption Event Candidate Without a Detected Host Galaxy at z = 0.995

We report multi-wavelength observations and characterization of the ultraluminous transient AT 2021lwx (ZTF20abrbeie; aka ``Barbie'') identified in the alert stream of the Zwicky Transient Facility (ZTF) using a Recommender Engine For Intelligent Transient Tracking (REFITT) filter on the ANTARES alert broker. From a spectroscopically measured redshift of 0.995, we estimate a peak observed pseudo-bolometric luminosity of log (L$_{\text{max}} / [\text{erg}/\text{s}]$) = 45.7 from slowly fading ztf-$\it{g}$ and ztf-$r$ light curves spanning over 1000 observer-frame days. The host galaxy is not detected in archival Pan-STARRS observations ($g > 23.3$ mag), implying a lower limit to the outburst amplitude of more than 5 mag relative to the quiescent host galaxy. Optical spectra from Lick and Keck Observatories exhibit strong emission lines with narrow cores from the H Balmer series and ultraviolet semi-forbidden lines of Si III] $\lambda$1892, C III] $\lambda$1909, and C II] $\lambda$2325. Typical nebular lines in AGN spectra from ions such as [O II] and [O III] are not detected. These spectral features, along with the smooth light curve that is unlike most AGN flaring activity, and the luminosity that exceeds any observed or theorized supernova, lead us to conclude that AT 2021lwx is most likely an extreme tidal disruption event (TDE). Modeling of ZTF photometry with MOSFiT suggests that the TDE was between a $\approx 14 M_{\odot}$ star and a supermassive black hole of mass $M_{\text{BH}} \sim$ $10^{8} M_{\odot}$. Continued monitoring of the still-evolving light curve along with deep imaging of the field once AT 2021lwx has faded can test this hypothesis and potentially detect the host galaxy.

==> AT2021lwx_TDE_Fit_Parameters.tex <==
\begin{deluxetable}{cccccc}[tph]
%\linespread{1.0}
%\setlength{\tabcolsep}{0.8pt} 
\tablecaption{Prior Distribution and Best Fits of physical parameters in the MOSFiT TDE model. \label{tab:tab2}}
\tablecolumns{6}
\tablewidth{0pt}
\tablehead{
\colhead{Parameter} & 
\colhead{Prior} & 
\colhead{Min}&
\colhead{Max}&
\colhead{Best Fit}& %\tablenotemark{${\dagger}$}
\colhead{Units}
}
\startdata
$M_{\text{BH}}$ & Log& $10^{5}$ & $5 \times 10^{8}$ & $8.23 \pm 0.03$ & M$_\odot$ \\
$M_{\star}$& Flat &0.01 & 100 & $14.28_{-1.65}^{+0.67}$& M$_\odot$ \\
$R_{ph0}$ & Log&$10^{-4}$& $10^{4}$& $2.34_{-0.22}^{+0.26}$& --\\
$T_{viscous}$ & Log & $10^{-3}$& $10^{5}$&$1.16_{-0.18}^{+0.12}$& day \\
\textit{b}& Flat & 0 & 2& $0.71_{-0.04}^{+0.03}$& --\\
$\epsilon$& Log & 0.0001&0.4&  $-1.01_{-0.06}^{+0.07}$& --\\
\textit{l}& Flat & 0 & 4 & $1.50_{-0.39}^{+0.28}$& --\\
$t_{\text{first fallback}}$&Flat& -500& 0 & $-72.52_{-7.54}^{+7.59}$& day\\
$n_{H host}$& Log & $10^{16}$&$10^{23}$ & $20.55_{-0.06}^{+0.05}$ & cm$^{-2}$\\
$\sigma$& Log & 0.001& 100&$ -0.69 \pm 0.02$&-- \\
\enddata
\tablecomments{$M_{\text{BH}}$ is the mass of the disrupting
black hole, $M_{\star}$ is the mass of the disrupted star, $R_{ph0}$ is he photosphere radius power-law constant, $T_{viscous}$ is the viscous timescale, \textit{b} is the scaled impact parameter, $\epsilon$ is the efficiency,  \textit{l} is the photosphere power-law exponent, $t_{\text{first fallback}}$ is the disruption time relative to the first detection, $n_{H host}$ is the column density in the host galaxy and $\sigma$ is the model uncertainty.} 
\end{deluxetable}
%the photosphere radius power-law constant, $T_{viscous}$ is the viscous
%timescale, \textit{b} is the scaled impact parameter, $\epsilon$ is the efficiency,  \textit{l} is the photosphere power-law exponent, $t_{\text{first fallback}}$ is the disruption time relative to the first detection, $n_{H host}$ is the column density in the host galaxy and $\sigma$ is the model uncertainty.}
%\tablecomments{$M_{\text{BH}}$ is the mass of the disrupting
%black hole, $M_{\star}$ is the mass of the disrupted star, $R_{ph0}$ is}

==> AT2021lwx_spectra_log.tex <==
\begin{deluxetable*}{lcccccccc}
\tablecaption{Log of AT 2021lwx Spectroscopic Observations}
\tablehead{
\colhead{UT Date} &
\colhead{Phase}  &
\colhead{Instrument} &
%\colhead{Blue Grism} &
%\colhead{Red Grating}  &
\colhead{Wavelength Range} &
\colhead{Resolution} &
\colhead{Exposure Time} &
\colhead{Airmass} \\
%\colhead{(YYYY MM DD)} &
\colhead{} &
\colhead{(days)} &
\colhead{} &
%\colhead{} &
%\colhead{} &
\colhead{(\AA)} &
\colhead{(\AA)} &
\colhead{(s)} &
\colhead{}
}
\startdata
2022 Jun 26.405   & \nodata & Kast       & 
3520--10700 & 6/6\tablenotemark{a} & 2430/2400\tablenotemark{a} & 1xx \\
2022 Sep 02.428   & \nodata & Kast       & 
3510--10700 & 6/6 & 2860/2800 & 1xx \\
2022 Sep 25.209   & \nodata & LRIS       & 
3040--10280 & 6/6 & 240/240 & 1xx \\
2022 Nov 25.216   & \nodata & LRIS       & 
3040--10320 & 6/6 & 660/600 & 1xx \\
\enddata
\tablenotetext{a}{Blue/red sides, respectively.}
\label{tab:lwxspec}
\end{deluxetable*}


==> EzGal_Mass_Limits.tex <==
\begin{deluxetable}{cccccc}[tph]
%\linespread{1.0}
%\setlength{\tabcolsep}{0.8pt} 
\tablecaption{Upper limit on host galaxy stellar mass \label{tab:mass_limits}}
\tablecolumns{3}
\tablewidth{0pt}
\tablehead{
\colhead{Age (Gyr)/$z_f$} & 
\multicolumn{2}{c}{Stellar mass (10$^{9}$ $M_\odot$)} 
}
\startdata
 & $\tau = $ 0.1 Gyr & $\tau =$ 1.0 Gyr \\
 \hline
0.1/1.02 & 0.03 & 0.03 \\
0.5/1.13 & 0.80 & 0.12 \\
1.0/1.28 & 6.95 & 0.29 \\
3.0/2.25 & 68.72 & 2.80\\
4.0/3.30 & 111.48 & 7.45 \\
\enddata
\tablecomments{Age refers to the age of the model at $z = $ 0.995 and $z_f$ refers to the corresponding formation redshift of the model.} 
\end{deluxetable}
